Building on Efficient Foundations: Effectively Training LLMs with Structured Feedforward Layers

State-of-the-art results in large language models (LLMs) often rely on scale, which becomes computationally expensive. This has sparked a research agenda to reduce these models' parameter counts and computational costs without significantly impacting their performance. Our study focuses on transformer-based LLMs, specifically targeting the computationally intensive feedforward networks (FFNs), which are less studied than attention blocks. We consider three structured linear parameterizations of the FFN using efficient low-rank and block-diagonal matrices. In contrast to many previous works that examined these approximations, our study i) explores these structures from a training-from-scratch perspective, ii) scales up to 1.3B parameters, and iii) is conducted within recent Transformer-based LLMs rather than convolutional architectures. We demonstrate that these structures can lead to actual computational gains in various scenarios, including online decoding when using a pre-merge technique. Additionally, we propose a novel training regime, called \textit{self-guided training}, aimed at improving the poor training dynamics that these approximations exhibit when used from initialization. Interestingly, the scaling performance of structured matrices is explored, revealing steeper curves in scaling training FLOPs, along with a favorable scaling trend in the overtraining regime. Specifically, we show that wide and structured networks can utilize training FLOPs more efficiently, with fewer parameters and lower loss than dense models at their optimal trade-off. Our code is available at \url{https://github.com/CLAIRE-Labo/StructuredFFN/tree/main}.

==> tables/complete/sgt.tex <==
\begin{table}[htbp]
\footnotesize
    \centering
    \captionof{table}{Performance when applying the self-guided training$^\clubsuit$ to Structured FFN with 32\% parameters in the first half of training. Model FLOPs are calculated on one sample with 1024 sequence length.}
    \begin{adjustbox}{max width=0.9\textwidth}
    \begin{tabular}{llllcHcccc}
    \toprule
    % \bf Architecture & \bf {Model size} & \bf {FFN size} & \bf {Model FLOPs (G)} & \bf {Tokens (B)} & \bf {Training steps} & \bf {Training FLOPs} & \bf Loss & \bf PPL \\ 
    \multirow{2}{*}{\bf Architecture} & \bf Model & \bf FFN & \bf Model & \multicolumn{3}{c}{\bf Training} &\multirow{2}{*}{\bf Loss} & \multirow{2}{*}{\bf PPL} \\
    \cmidrule{5-7}
    & \bf Size (M) & \bf Size (M) & \bf FLOPs (G) & \bf Tokens (B) & \bf Steps (K) & \bf {FLOPs}& & \\

    \midrule
        \bf Transformer-s & 110 & 56.62 & 262.9&  2.2 & 4K & 1.69e+18 & 
        3.2569 & 25.97 \\
        \midrule
        \hspace{0.5em} \lowrank{}  & \multirow{2}{2em}{73.95} & \multirow{2}{2em}{20.94} & \multirow{2}{2em}{189.8} &  2.2 & 4K & 1.22e+18 & 
        3.3748 & 29.22 \\
        % \hspace{0.5em} \lowrank{} &  &  &  & 3.0 \iffalse 3.04 \fi & 6K & 1.69e+18 & 3.2928 & 26.92 \\
        % \hspace{0.5em} \lowrank{}$^\diamondsuit$ (slower) & 0.325x & 4196 & 1.56e+18 & 
        % 3.3287 & 27.90 \\
        \hspace{0.5em} \lowrank{}$^\clubsuit$ & & & & 2.2 & 4K & 1.39e+18 &
        3.3329 & \bf 28.02 \\
        % \hspace{0.5em} \lowrank{}$^\diamondsuit$ &  &  & & 2.2 & 5K & 1.69e+18 & 3.2866 & \bf 26.75\\
        \midrule
        \hspace{0.5em} \blockrank{}  & \multirow{2}{2em}{73.95} & \multirow{2}{2em}{20.94} & \multirow{2}{2em}{189.8} &  2.2 & 4K & 1.22e+18 & 
        3.3731 & 29.17 \\
        % \hspace{0.5em} \blockrank{} &  &  &  & 3.0 \iffalse 3.04 \fi & 6K & 1.69e+18 &
        % 3.2982 &27.06 \\
        \hspace{0.5em} \blockrank{}$^\clubsuit$ &  &  & & 2.2 & 4K & 1.39e+18 &
        3.3338 & \bf 28.04\\
        % \hspace{0.5em} \blockrank{}$^\diamondsuit$ &  &  & & 2.2 & 5K & 1.69e+18&
        % 3.2856 & \bf 26.73 \\
        \midrule
        \hspace{0.5em} \shufflelinear{} & \multirow{2}{2em}{73.95} & \multirow{2}{2em}{20.94} & \multirow{2}{2em}{189.8} &  2.2 & 4K & 1.22e+18 & 
        3.3994 & 29.95 \\
        % \hspace{0.5em} \shufflelinear{}  &  &  &  & 3.0 \iffalse 3.04 \fi & 6K & 1.69e+18 &
        % 3.3218 & 27.71\\
        \hspace{0.5em} \shufflelinear{}$^\clubsuit$ & & & & 2.2 & 4K & 1.39e+18 &
        3.3583 & \bf 28.74\\
        % \hspace{0.5em} \shufflelinear{}$^\diamondsuit$ &  &  & & 2.2 & 5K & 1.69e+18&
        % 3.3011 & \bf 27.14 \\
        \midrule
        \bf Transformer-m & 335.08 & 201.33 & 788.7 & 6.7 & 13K & 1.55e+19 & 
        2.9062 & 18.29\\
        \midrule
        \hspace{0.5em} \lowrank{}  & \multirow{2}{2em}{202.43} & \multirow{2}{2em}{68.68} & \multirow{2}{2em}{517.0} & 6.7 & 13K & 1.01e+19 & 
        3.0251 & 20.60 \\
        % \hspace{0.5em} \lowrank{} &  &  &  & 10.2 & 19K \iffalse 19454 \fi & 1.54e+19 & 
        % 2.9359 & 18.84 \\
        \hspace{0.5em} \lowrank{}$^\clubsuit$ & & &  & 6.7 & 
        13K & 1.21e+19 & 
        2.9907 & \bf 19.90 \\
        % \hspace{0.5em} \lowrank{}$^\diamondsuit$ &  &  &  &  6.7 & 18K & 1.55e+19 & 
        % 2.9310 & \bf 18.75 \\
        \midrule
        \hspace{0.5em} \blockrank{}  & \multirow{2}{2em}{198.67} & \multirow{2}{2em}{64.91} & \multirow{2}{2em}{509.3} & 6.7 & 13K & 1.00e+19 & 
        3.0371 & 20.85\\
        % \hspace{0.5em} \blockrank{} &  &  &  & 10.4 & 20K & 1.55e+19 & 
        % 2.9491& 19.09\\
        \hspace{0.5em} \blockrank{}$^\clubsuit$ &  & & &  6.7  & 13K & 1.19e+19 & 
        3.0008 & \bf 20.10\\
        % \hspace{0.5em} \blockrank{} $^\diamondsuit$  &  &  &  & 6.7 & 18K\iffalse 17890 \fi & 1.55e+19 & 
        % 2.9420 & \bf 18.95 \\
         \midrule
        \hspace{0.5em} \shufflelinear{}  & \multirow{2}{2em}{202.43} & \multirow{2}{2em}{68.68} & \multirow{2}{2em}{517.0} & 6.7 & 13K &  1.01e+19 & 
        3.0501 & 21.12 \\
        % \hspace{0.5em} \shufflelinear{} &  &  &  & 10.2 & 19K \iffalse 19454 \fi & 1.54e+19 & 
        % 2.9627  & 19.35 \\
        % \hdashline
        \hspace{0.5em} \shufflelinear{}$^\clubsuit$ & && & 6.7 & 
        13K & 1.21e+19 & 
        3.0135 & \bf 20.36\\
        % \hspace{0.5em} \shufflelinear{}$^\diamondsuit$ &  &  &  &  6.7 & 18K & 1.55e+19 & 
        % 2.9525 & \bf 19.15 \\
        \iffalse
        \midrule
       \bf Transformer-l & 729.11 & 452.98 & 1646.9 & 14.6 & 28K & 7.03e+19 & 
        2.6594 & 14.29\\
        \midrule
        \hspace{0.5em} \lowrank{}  & \multirow{2}{2em}{430.66} & \multirow{2}{2em}{154.53} & \multirow{2}{2em}{1035.6} & 14.6 & 28K & 4.42e+19 & 
        2.7527 & 15.69 \\
        \hspace{0.5em} \lowrank{} & & & & 23.3 & 44K & 7.03e+19 & 
        2.6917& 14.76\\
        \hdashline
        \hspace{0.5em} \lowrank{}$^\diamondsuit$ & 430.66 & 154.53 &1035.6 & 14.6 & 39K & 7.01e+19 & 
        2.6850 & 14.66\\
        \midrule
        \hspace{0.5em} \blockrank{}  & \multirow{2}{2em}{430.66} & \multirow{2}{2em}{154.53} & \multirow{2}{2em}{1035.6} & 14.6 & 28K & 4.42e+19 & 
        2.7570 & 15.75\\
        \hspace{0.5em} \blockrank{} & & & & 23.3 & 44K & 7.03e+19 & 
        2.6946 & 14.80\\
        \hdashline
        \hspace{0.5em} \blockrank{}$^\diamondsuit$ & 430.66 & 154.53 &1035.6 & 14.6 & 39K & 7.01e+19 & 
        2.6941 & 14.79\\
         \midrule
        \hspace{0.5em} \shufflelinear{}  & \multirow{2}{2em}{430.66} & \multirow{2}{2em}{154.53} & \multirow{2}{2em}{1035.6} & 14.6 & 28K & 4.42e+19 & 
        2.7735 & 16.01 \\
        \hspace{0.5em} \shufflelinear{} & & & & 23.3 & 44K & 7.03e+19 & 
        2.7053 & 14.96\\
        \hdashline
        \hspace{0.5em} \shufflelinear{}$^\diamondsuit$ & 430.66 & 154.53 &1035.6 & 14.6 & 39K & 7.01e+19 & 
        2.7104 & 15.04\\
        \midrule
       \bf Transformer-xl & 1274.14 & 805.31 & 2814.3 & 25.5 & 49K & 2.10e+20 &  2.5226 & 12.46 \\
       \midrule
        \hspace{0.5em} \lowrank{}  & \multirow{2}{2em}{743.56} & \multirow{2}{2em}{274.73} & \multirow{2}{2em}{1727.7} & 25.5 & 49K & 1.29e+20 & 2.6062 & 13.55 \\
        \hspace{0.5em} \lowrank{} & & & & 41.5 & 79K & 2.10e+20 & 
        2.5464 & 12.76\\
        \hdashline
        \hspace{0.5em} \lowrank{}$^\diamondsuit$ & 743.56 & 274.73 & 1727.7 & 25.5 & 70K & 2.10e+20 & 
        2.5539 & 12.86 \\
        \midrule
        \hspace{0.5em} \blockrank{}  & \multirow{2}{2em}{728.49} & \multirow{2}{2em}{259.65} & \multirow{2}{2em}{1696.8} & 25.5 & 49K & 1.27e+20 & 2.6204 & 13.74 \\
        \hspace{0.5em} \blockrank{} & & & & 42.2 & 80K & 2.10e+20 & 
        -& -\\
        \hdashline
        \hspace{0.5em} \blockrank{}$^\diamondsuit$ & 728.49 & 259.65 & 1696.8 & 25.5 & 71K & 2.10e+20 & 
        2.5637 & 12.98\\
        \midrule
        \hspace{0.5em} \shufflelinear{} & \multirow{2}{2em}{743.56} & \multirow{2}{2em}{274.73} & \multirow{2}{2em}{1727.7} & 25.5 & 49K & 1.29e+20 & 2.6254 & 13.81 \\
        \hspace{0.5em} \shufflelinear{} & & & & 41.5 & 79K & 2.10e+20 & 
        2.5623 & 12.97\\
        \hdashline
        \hspace{0.5em} \shufflelinear{}$^\diamondsuit$ & 743.56 & 274.73 & 1727.7 & 25.5 & 70K & 2.10e+20 & 
        2.5678 & 13.03\\
        \midrule
        \fi
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:sgt_complete}
\end{table}
\vspace{1\baselineskip}

==> tables/sgt_ablation.tex <==
\begin{table}[htbp]
\footnotesize
\caption{}
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lll}
    \toprule
    \bf Method & \bf {Steps} & \bf {Training FLOPs} & \bf Loss & \bf PPL \\ 
    \midrule
        \hspace{0.5em} Direct decomposition & & &
        \hspace{0.5em} Incrementally decrease rank
        \hspace{0.5em} LowRank$^\diamondsuit$ & 2.2 & 4196 & 
        &  \\
        \midrule
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:sgt_ablation}
\end{table}
